The Locus Story of a Rocking Camel in a Medical Center in the City of Freistadt

We give an example of automated geometry reasoning for an imaginary classroom project by using the free software package GeoGebra Discovery. The project is motivated by a publicly available toy, a rocking camel, installed at a medical center in Upper Austria. We explain how the process of a false conjecture, experimenting, modeling, a precise mathematical setup, and then a proof by automated reasoning could help extend mathematical knowledge at secondary school level and above.

==> eptcsdata.tex <==
\providecommand{\firstpage}{132}
\providecommand{\publicationstatus}{P. Quaresma and Z. Kov{\'a}cs (Ed.): Automated Deduction\\ in Geometry 2023 (ADG 2023).\\
EPTCS 398, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.398.16}{10.4204/EPTCS.398.16}}
\pdfoutput=1

